Fast Approximation in Subspaces by Doubling Metric Decomposition

In this paper we propose and study a new complexity model for approximation algorithms. The main motivation are practical problems over large data sets that need to be solved many times for different scenarios, e.g., many multicast trees that need to be constructed for different groups of users. In our model we allow a preprocessing phase, when some information of the input graph $G=(V,E)$ is stored in a limited size data structure. Next, the data structure enables processing queries of the form ``solve problem A for an input $S\subseteq V$''. We consider problems like {\sc Steiner Forest}, {\sc Facility Location}, {\sc $k$-Median}, {\sc $k$-Center} and {\sc TSP} in the case when the graph induces a doubling metric. Our main results are data structures of near-linear size that are able to answer queries in time close to linear in $|S|$. This improves over typical worst case reuniting time of approximation algorithms in the classical setting which is $\Omega(|E|)$ independently of the query size. In most cases, our approximation guarantees are arbitrarily close to those in the classical setting. Additionally, we present the first fully dynamic algorithm for the Steiner tree problem.

==> a1_jump.tex <==
\section{Implementing the $\jump$ operation}
In this section we show how to implement the $\jump$ operation in $O(\log \log n)$ time by combining the y-Fast Tree data structure~\cite{Willard84,Willard86} with the path decomposition technique~\cite{st81}. The y-Fast Trees can be used to answer predecessor queries on a polynomially bounded universe in time $O(\log \log n)$ using linear space. We use this structure to store the information of levels on some sub paths of the tree. 

\begin{lemma}
The tree $\hat{\cT}$ can be augmented by $O(n)$ additional information so that $\jump$ operation can be performed in $O(\log\log n)$ time.
\end{lemma}

\begin{proof}
Define $\size(v)$ to be the size of the subtree rooted at $v$. In the path decomposition we classify the edges $(v,w)$ in heavy - when $2\size(v)>\size(w)$ - and light otherwise. The paths for the decomposition are defined as connected by heavy edges sets of vertices. Note that when we are going from any leaf to the root we pass no more then $\log n$ light edges, so we do not pass more then $\log n$ paths as well. We define the beginning of the path to be the highest vertex on it, and let depth $d(\pi)$ of the path $\pi$ be it's order on the way from the root. Let us fix $x = \lceil \log \log n\rceil$. In order to represent the tree we store:
\begin{itemize}
\item each path in y-Fast Tree where the keys are the levels of the vertices,
\item for each vertex $v$ on the path a pointer $p(v)$ to a data structure representing the path,
\item for each path $\pi$ a pointer $p(\pi)$ to the next path on the way to the root, 
\item for each path $\pi$ a pointer $s(\pi)$ to the path that we encounter as $x2^{d(\pi) \mod x}$'th one on the way to the root, or to the root if no such path exists.
\end{itemize}

The jump operation is now realized in two steps. In the first we find the lowest path $\pi$ on the way from $v$ to the root such that $\level(p(\pi))>j$. Then we can use y-Fast Tree associated with $\pi$ to find the predecessor of $j$ on $\pi$ in time $O(\log \log n)$, which is returned from by the $\jump$ operation. In order to find the path $\pi$ we simulate a binary search using the pointers $p$ and $s$. This search starts at $\pi = p(v)$ and works in the following steps:
\begin{itemize}
\item go up to $p(\pi)$ till you find $\pi$ such that $d(\pi) \mod x = x-1$, 
\item repeat till you find $\pi$ such that $d(\pi) \mod x = 0$,
\begin{itemize}
\item if $\level(p(s(\pi))) \le j$ go up to $p(s(\pi))$,
\item else go up to $p(\pi)$, 
\end{itemize}
\item go up to $p(\pi)$ till you find $\pi$ such that $\level(p(\pi))>j$.
\end{itemize}

First of all note that going up to $s(\pi)$ does not change the depth of the path modulo $x$, whereas going up to $p(\pi)$ decreases it by $1$. Moreover, the middle step of the search starts when $d(\pi) \mod x = x-1$, so $x2^{d(\pi) \mod x} \ge \log n$ and finishes when $d(\pi) \mod x = 0$. Hence, $d(\pi) mod x$ ranges from $x-1$ down to $0$ and as every time we are looking at a path $x2^{d(\pi) \mod x}$ far apart we perform a binary search times $x$. Now, when the middle step finishes we are at distance at most $x$ from the node we are looking for, so the last step is executed at most $x$ times. Moreover, in the first step we went up at most $x$ nodes up as well, so the total time needed to execute $\jump$ is bounded by $O(\log \log n)$.
\end{proof}

